On the acceleration of forward-backward splitting via an inexact Newton method

We propose a Forward-Backward Truncated-Newton method (FBTN) for minimizing the sum of two convex functions, one of which smooth. Unlike other proximal Newton methods, our approach does not involve the employment of variable metrics, but is rather based on a reformulation of the original problem as the unconstrained minimization of a continuously differentiable function, the forward-backward envelope (FBE). We introduce a generalized Hessian for the FBE that symmetrizes the generalized Jacobian of the nonlinear system of equations representing the optimality conditions for the problem. This enables the employment of conjugate gradient method (CG) for efficiently solving the resulting (regularized) linear systems, which can be done inexactly. The employment of CG prevents the computation of full (generalized) Jacobians, as it requires only (generalized) directional derivatives. The resulting algorithm is globally (subsequentially) convergent, $Q$-linearly under an error bound condition, and up to $Q$-superlinearly and $Q$-quadratically under regularity assumptions at the possibly non-isolated limit point.

==> TeX/Alg/CG.tex <==
\begin{algorithmic}[1]
% \renewcommand\algorithmicrequire{\textfillwidthof[l]{\textsc{Output}}{\textsc{Input}}}%
% \renewcommand\algorithmicensure{\textsc{Output}}%
	\Require{%
		\(A\in\sym_{++}(\R^n)\),~
		\(b\in\R^n\),~
		precision \(\varepsilon\geq0\)
	}
	\Ensure{%
		\(x\in\R^n\) such that \(\|Ax-b\|\leq\varepsilon\)
	}
	\Initialize{%
		\(x\gets 0\),~
		\(e\gets b\),~
		\(p\gets e\)
	}
	\While{~\(\|e\|>\varepsilon\)~}
		\def\myVar#1{\fillwidthof[l]{\alpha}{#1}}
		\State\label{step:pAp}\(
			\myVar\alpha
		{}\gets{}
			\|e\|^2 / \innprod{p}{Ap}
		\)
		\State\(
			\myVar x
		{}\gets{}
			x + \alpha p
		\),~~
		\(
			e^+
		{}\gets{}
			e - \alpha Ap
		\)
		\State\(
			\myVar p
		{}\gets{}
			e^+ + \bigl(\nicefrac{\|e^+\|}{\|e\|}\bigr)^2p
		\)
		\State\(
			\myVar e
		{}\gets{}
			e^+
		\)
	\EndWhile{}
\end{algorithmic}


==> TeX/Alg/FBN.tex <==
\begin{algorithmic}[1]
	\Require{%
		\(\gamma\in(0,\nicefrac{1}{L_f})\);~
		\(\sigma\in(0,\nicefrac12)\);~
		\(\bar\eta,\zeta\in(0,1)\);~
		\(\rho\in(0,1]\);~
		\(x_0\in\R^n\)
	}
	\Initialize{%
		\(k\gets 0\)
	}
% 	\def\myVar#1{\fillwidthof[l]{\alpha}{#1}}
	\State\label{step:FBN:1}%
		\(
			\delta_k\gets\zeta\|\nabla\varphi_\gamma(x^k)\|
		\),~
		\(
			\eta_k\gets\min\set{\bar\eta,\,\|\nabla\varphi_\gamma(x^k)\|^\rho}
		\),~
		\(
			\varepsilon_k\gets\eta_k\|\nabla\varphi_\gamma(x^k)\|
		\)
	\State
		Select \(H_k\in\hat\partial^2\varphi_\gamma(x^k)\)
	\State\label{step:FBN:CG}%
		Apply CG \Cref{alg:CG} to find an \(\varepsilon_k\)-approximate solution \(d^k\) to
		\[
			\bigl[H_k+\delta_k\I\bigr]d^k
		{}\approx{}
			-\nabla\varphi_\gamma(x^k)
		\]
	\State\label{step:FBN:LS}%
		Let \(\tau_k\) be the maximum in \(\set{2^{-i}}[i\in\N]\) such that the point \(x^{k+\nicefrac12}=x^k+\tau_kd^k\) satisfies
		\begin{equation}\label{eq:LS}
			\varphi_\gamma(x^{k+\nicefrac12})
		{}\leq{}
			\varphi_\gamma(x^k)
			{}+{}
			\sigma\tau_k\innprod{\nabla\varphi_\gamma(x^k)}{d^k}
		\end{equation}
		\State\label{step:FBN:variant}%
			{\color{MidnightBlue}\bf Basic scheme:}  \(x^{k+1}\gets x^{k+\nicefrac12}\),~
			or~
			{\color{MidnightBlue}\bf\textit{``global''} variant:} \(x^{k+1}\gets\FB{x^{k+\nicefrac12}}\)%
	\State
		\(k\gets k+1\) and go to \cref{step:FBN:1}
\end{algorithmic}


==> TeX/Text/Algorithm/Global.tex <==
In this subsection we specialize the results to the global variant of \Cref{alg:FBN}, and show that the additional proximal gradient step ensures the same complexity estimates of FBS.
\ifpanoc
\else
	\begin{thm}
		Consider the sequence \(\seq{x^k}\) generated by the global variant of \Cref{alg:FBN}.
		Suppose that \(\varphi\) has bounded level sets, and let \(R>0\) be such that
		\(
			\lev_{\leq\varphi(x_0)}\varphi
		{}\subseteq{}
			\cball{x_\star}{R}
		\)
		for some \(x_\star\in\argmin\varphi\).
		
		If \(\varphi(x^0)-\varphi_\star\geq\frac{1}{\gamma}R^2\), then 
		\begin{subequations}
			\begin{align}\label{eq:FirstStep}
				\varphi(x^1)-\varphi_\star
			{}\leq{} &
				\frac{1}{2\gamma}R^2,
			\shortintertext{%
				otherwise,
			}
			\label{eq:kStep}
				\varphi(x^k)-\varphi_\star
			{}\leq{} &
				\frac{1}{\gamma(k+2)}
				2R^2
			\quad
				\text{for any \(k\in\N\).}
			\end{align}
		\end{subequations}
		\begin{proof}
			From \cref{thm:FBE-Moreau} we have that \(\FBE\) is upper bounded by the convex function \(\varphi^\gamma\).
			Combining this with \eqref{eq:SD0} we obtain that
			\(
				\varphi(x^{j+1})
			{}\leq{}
				\varphi^\gamma(x^j)
			\)
			for all \(j\in\N\).
			The rest of the proof is similar to that of \cite[Thm. 4]{nesterov2013gradient}.
			
			In particular we have
			\begin{align*}
				\varphi(x^{j+1})
			{}\leq{} &
				\varphi^\gamma(x^j)
			{}={}
				\min_{w\in\R^n}\set{
					\varphi(x)
					{}+{}
					\tfrac{1}{2\gamma}
					\|w-x^j\|^2
				}
			\\
			{}\leq{} &
				\min_{\alpha\in[0,1]}\set{
					\varphi(\alpha x_\star+(1-\alpha)x^j)
					{}+{}
					\tfrac{1}{2\gamma}
					\|\alpha(x^j-x_\star)\|^2
				}
			\\
			{}\leq{} &
				\min_{\alpha\in[0,1]}\set{
					\varphi(x^j)
					{}-{}
					\alpha(\varphi(x^j)-\varphi_\star)
					{}+{}
					\tfrac{1}{2\gamma}(\alpha R)^2
				},
			\end{align*}
			where the last inequality follows by convexity of \(\varphi\).
			
			If
			\(
				\varphi(x^0)-\varphi_\star
			{}\geq{}
				\frac{1}{\gamma}R^2
			\),
			then the minimizer of the latter problem for \(j=0\) is \(\alpha=1\) and we obtain \eqref{eq:FirstStep}.
			
			Otherwise, the minimizer is
			\(
				\alpha
			{}={}
				\gamma\frac{\varphi(x^j)-\varphi_\star}{R^2}
			{}\leq{}
				\gamma\frac{\varphi(x^0)-\varphi_\star}{R^2}
			{}\leq{}
				1
			\)
			and we obtain
			\[
				\varphi(x^{j+1})
			{}\leq{}
				\varphi(x^j)
				{}-{}
				\frac{
					\gamma(\varphi(x^j)-\varphi_\star)^2
				}{
					2R^2
				}.
			\]
			Letting \(\lambda_j=\frac{1}{\varphi(x^j)-\varphi_\star}\), which is increasing as it follows from \eqref{eq:SD}, the latter inequality is expressed as
			\begin{align*}
				\frac{1}{\lambda_{j+1}}
			{}\leq{} &
				\frac{1}{\lambda_j}
				{}-{}
				\frac{\gamma}{2R^2\lambda_j^2}.
			\shortintertext{%
				Multiplying both sides by \(\lambda_j\lambda_{j+1}\) and rearranging,
			}
				\lambda_{j+1}
			{}\geq{} &
				\lambda_j
				{}+{}
				\frac{\gamma}{2R^2}
				\frac{\lambda_{j+1}}{\lambda_j}
			{}\geq{}
				\lambda_j
				{}+{}
				\frac{\gamma}{2R^2}.
			\shortintertext{%
				Telescoping the outer inequality for \(j=0,\ldots,k-1\) we obtain
			}
				\lambda_k
			{}\geq{} &
				\lambda_0
				{}+{}
				\frac{\gamma}{2R^2}k
			{}\geq{}
				\frac{\gamma}{2R^2}(k+2)
			\end{align*}
			where the last inequality follows from the fact that
			\(
				\varphi(x^0)-\varphi_\star
			{}\leq{}
				\frac{1}{\gamma}R^2
			\).
			Rearranging, we arrive at \eqref{eq:kStep}.
		\end{proof}
	\end{thm}

	\begin{thm}%
		Suppose that \(\varphi\) satisfies the error bound \eqref{eq:EB} with constant \(m>0\).
		Then, the following bounds hold for the iterates generated by the global variant of \Cref{alg:FBN}.
		\begin{proof}
			We have that
			\(
				\varphi(x^{k+1})
			{}\leq{}
				\varphi(x^{k+\nicefrac12})
			{}\leq{}
			\)
			From \cref{thm:EB} it follows that

		\end{proof}
	\end{thm}
	\begin{thm}\label{thm:linear}%
		Suppose that \(f\) is strongly convex.
		Then, the following bounds hold for the iterates generated by the global variant of \Cref{alg:FBN}
		\begin{subequations}
			\begin{align}
			\label{eq:strC1}
				\varphi(x^k)-\varphi_\star
			{}\leq{} &
				\bigr(
					{%\color{blue}
						1-\gamma\mu_f(2-\gamma L_f)
					}
				\bigl)^k
				\bigl(
					\varphi(x^0)-\varphi_\star
				\bigr)
			\\
			\label{eq:strC2}
				\|x^k-x_\star\|^2
			{}\leq{} &
				\tfrac{1-\gamma\mu_f}{\gamma\mu_f}
				\bigr(
					1-\gamma\mu_f(2-\gamma L_f)
				\bigl)^k
				\|x^{\nicefrac12}-x_\star\|^2.
			\end{align}
	% 		\hl{Note that $1-\gamma\mu_f(2-\gamma L_f)<1-\gamma\mu_f<(1+\gamma\mu_f)^{-1}=$ previous coeff.}
		\end{subequations}
		\begin{proof}
			Since \(x^{k+1}=\T(x^{k+\nicefrac12})\), the following inequalities hold:
			\begin{align*}
				\|\Res(x^{k+\nicefrac12})\|^2
			{}\overrel[\geq]{\ref{thm:ErrorBound}}{} &
				\tfrac{
					2\mu_f
				}{
					{%\color{red}
						1-\gamma\mu_f(2-\gamma L_f)
					}
				}
				\bigl(
					\varphi(x^{k+1})
					{}-{}
					\varphi_\star
				\bigr)
			\shortintertext{and}
				\varphi(x^{k+1})
			{}\overrel*[\leq]{\eqref{eq:SDFBS}}{} &
				\varphi(x^{k+\nicefrac12})
				{}-{}
				\gamma\tfrac{2-\gamma L_f}{2}
				\|\Res(x^{k+\nicefrac12})\|^2
			{}\overrel*[\leq]{\eqref{eq:descent}}{}
				\varphi(x^k)
				{}-{}
				\gamma\tfrac{2-\gamma L_f}{2}
				\|\Res(x^{k+\nicefrac12})\|^2.
			\end{align*}
			Plugging the first one in the second one we obtain
			\begin{align*}
				\varphi(x^{k+1})-\varphi_\star
			{}\leq{} &
				\varphi(x^k)-\varphi_\star
				{}-{}
				\tfrac{
					\gamma\mu_f(2-\gamma L_f)
				}{
					{%\color{red}
						1-\gamma\mu_f(2-\gamma L_f)
					}
				}
				\bigl(
					\varphi(x^{k+1})
					{}-{}
					\varphi_\star
				\bigr)
			\shortintertext{%
				thus,
			}
				\bigl(
					\varphi(x^{k+1})
					{}-{}
					\varphi_\star
				\bigr)
			{}\leq{} &
				\bigr(
					1-\gamma\mu_f(2-\gamma L_f)
				\bigl)
				\bigl(
					\varphi(x^k)-\varphi_\star
				\bigr)
			\end{align*}
			which proves \eqref{eq:strC1}.
			In particular,
			\begin{align*}
				\varphi(x^{k+1})-\varphi_\star
			{}\leq{} &
				\bigr(
					1-\gamma\mu_f(2-\gamma L_f)
				\bigl)^k
				\bigl(
					\varphi(x^1)-\varphi_\star
				\bigr)
			\shortintertext{
				and since \(x^1=\T(x^{\nicefrac12})\), \cref{thm:cost_leq_dist} yields
			}
			{}\leq{} &
				\bigr(
					1-\gamma\mu_f(2-\gamma L_f)
				\bigl)^k
				\tfrac{1-\gamma\mu_f}{2\gamma}
				\left(
					1
					{%\color{red}
						{}-{}
						\gamma\mu_f
						\tfrac{
							2-\gamma L_f
						}{
							1-(\gamma\mu_f)(\gamma L_f)
						}
					}
				\right)
				\|x^{\nicefrac12}-x_\star\|^2
			\\
			{}\leq{} &
				\tfrac{1-\gamma\mu_f}{2\gamma}
				\bigr(
					1-\gamma\mu_f(2-\gamma L_f)
				\bigl)^{k+1}
				\|x^{\nicefrac12}-x_\star\|^2.
			\end{align*}
			We may now use \cref{thm:cost_geq_dist} to lower bound the first term and \eqref{eq:strC2} follows.
	% 		\begin{align*}
	% 			\|x^{k+1}-\varphi_\star\|
	% 		{}\leq{} &
	% 			\tfrac{1-\gamma\mu_f}{\gamma\mu_f}
	% 			\bigr(
	% 				1-\gamma\mu_f(2-\gamma L_f)
	% 			\bigl)^{k+1}
	% 			\|x^{\nicefrac12}-x_\star\|^2.
	% 		\end{align*}
		\end{proof}
	\end{thm}
\fi


==> TeX/Text/Proof_ProxAlg.tex <==
Before proving \Cref{thm:ErrorBounds} we first state an ancillary fact related to FBS.

% \todo{While it doesn't seem to extend \cite[Lem. 2.3]{beck2009fast} for strongly convex \(f\), as previously declared}%
The following proposition tightens the bound in \cite[Thm. 2.2.7]{nesterov2003introductory} and extends its validity to arbitrary convex \(g\), as opposed to indicators of convex sets.
\begin{prop}\label{thm:ProxIneq}%
	Let \(\gamma>0\) be fixed.
	Then, for all \(x,y\in\R^n\) it holds that
	\begin{equation}\label{eq:ProxIneq}
		\varphi(y)
	{}\geq{}
		\varphi(\bar x)
		{}+{}
		\tfrac{1}{2\gamma}\|y-\bar x\|^2
		{}-{}
		\tfrac{1-\gamma\mu_f}{2\gamma}\|x-y\|^2
		{%\color{red}
			{}+{}
			\tfrac{1-\gamma L_f}{2\gamma}\|x-\bar x\|^2
		}
	\end{equation}
	where \(\bar x\coloneqq\T(x)\).
	\begin{proof}
		Replacing the minimizer \(\bar x\) in \eqref{eq:FBEmin} yields the identity
		\begin{equation}\label{eq:FBE2}
			\FBE(x)
		{}={}
			f(x)
			{}+{}
			\innprod{\nabla f(x)}{\bar x-x}
			{}+{}
			g(\bar x)
			{}+{}
			\tfrac{1}{2\gamma}\|x-\bar x\|^2.
		\end{equation}
		Now,
		\begin{qedalign*}
			\varphi(y)
		{}\geq{} &
			\smashoverbracket{
				f(x)
				{}+{}
				\innprod{\nabla f(x)}{y-x}
				{}+{}
				\tfrac{\mu_f}{2}\|x-y\|^2
			}{
				\leq f(y)
				~~\text{(cf. \eqref{eq:LipBound})}
			}
			{}+{}
			\smashoverbracket{
				g(\bar x)
				{}+{}
				\innprod{
					\underbracket{
						\tfrac1\gamma(x-\bar x)-\nabla f(x)
					}_{
						\in\partial g(\bar x)
					~~\text{(cf. \eqref{eq:FBCharacterization})}
					}
				}{
					y-\bar x
				}
			}{
				\leq g(y)
			}
		\\
		{}={} &
			f(x)
			{}+{}
			\innprod{\nabla f(x)}{\bar x-x}
			{}+{}
			\tfrac{\mu_f}{2}\|x-y\|^2
			{}+{}
			g(\bar x)
			{}+{}
			\tfrac1\gamma
			\innprod{
				x-\bar x
			}{
				y-\bar x
			}
		\shortintertext{%
			expanding the rightmost inner product into three squares (see \eg \cite[Lem. 2.12]{bauschke2017convex})
		}
		{}={} &
			f(x)
			{}+{}
			\innprod{\nabla f(x)}{\bar x-x}
			{}-{}
			\tfrac{1-\gamma\mu_f}{2\gamma}\|x-y\|^2
			{}+{}
			g(\bar x)
			{}+{}
			\tfrac{1}{2\gamma}\|x-\bar x\|^2
			{}+{}
			\tfrac{1}{2\gamma}\|y-\bar x\|^2
		\\
		{}\overrel{\eqref{eq:FBE2}}{} &
			\FBE(x)
			{}-{}
			\tfrac{1-\gamma\mu_f}{2\gamma}\|x-y\|^2
			{}+{}
			\tfrac{1}{2\gamma}\|y-\bar x\|^2
		\\
		{}\overrel[\geq]{\ref{thm:geq}}{} &
			\varphi(\bar x)
			{}+{}
			{%\color{red}
				\tfrac{1-\gamma L_f}{2\gamma}\|x-\bar x\|^2
			}
			{}-{}
			\tfrac{1-\gamma\mu_f}{2\gamma}\|x-y\|^2
			{}+{}
			\tfrac{1}{2\gamma}\|y-\bar x\|^2.
		\end{qedalign*}
	\end{proof}
\end{prop}

% \begin{appendixproof}{thm:ErrorBounds}%
\begin{proof}{thm:ErrorBounds}%
	\begin{proofitemize}
	\item\ref{thm:cost_geq_dist}
		Follows from the subgradient inequality, since \(0\in\partial\varphi(x_\star)\) and \(\mu_\varphi\geq\mu_f\).
	\item\ref{thm:ErrorBound}~
		As functions of the sole variable \(y\), the left-hand side in \eqref{eq:ProxIneq} is pointwise larger than the right-hand side, thus the inequality holds for the respective minima.
		The minimum on the left-hand side is \(\varphi_\star\), while that on the right-hand side --- which is strongly convex quadratic --- is attained at
		\(
			y
		{}={}
			x
			{}-{}
			\tfrac{1}{\gamma\mu_f}
			(x-\bar x)
		{}={}
			x
			{}-{}
			\tfrac{1}{\mu_f}\Res(x)
		\).
		Replacing this value in the right-hand side of \eqref{eq:ProxIneq} yields the sought inequality.
	\item\ref{thm:cost_leq_dist}
		We have
		\begin{align*}
			\FBE(x)
		{}\overrel{\eqref{eq:FBEmin}}{} &
			\min_{w\in\R^n}\set{
				f(x)+\innprod{\nabla f(x)}{w-x}+\tfrac{1}{2\gamma}\|w-x\|^2
				{}+{}
				g(w)
			}
		\\
		{}\leq{} &
			f(x)+\innprod{\nabla f(x)}{x_\star-x}
			{}+{}
			\tfrac{1}{2\gamma}\|x_\star-x\|^2
			{}+{}
			g(x_\star)
		\\
		{}\overrel[\leq]{\eqref{eq:LipBound}}{} &
			f(x_\star)-\tfrac{\mu_f}{2}\|x-x_\star\|^2
			{}+{}
			\tfrac{1}{2\gamma}\|x_\star-x\|^2
			{}+{}
			g(x_\star)
		{}={}
			\varphi_\star
			{}+{}
			\tfrac{1-\gamma\mu_f}{2\gamma}\|x_\star-x\|^2.
		\end{align*}
		Combining this inequality with \cref{thm:geq}, we obtain
		\begin{align*}
			\varphi(\bar x)-\varphi_\star
		{}\leq{} &
			\tfrac{1-\gamma\mu_f}{2\gamma}\|x_\star-x\|^2
			{%\color{red}
				{}-{}
				\gamma\tfrac{1-\gamma L_f}{2}\|\Res(x)\|^2
			}
		\\
		{}\leq{} &
			\tfrac{1-\gamma\mu_f}{2\gamma}\|x_\star-x\|^2
				{%\color{red}
					{}-{}
					\gamma\tfrac{1-\gamma L_f}{2}
				\tfrac{
					2\mu_f
				}{
					1-\gamma\mu_f(2-\gamma L_f)
				}
				\bigl(
					\varphi(\bar x)
					{}-{}
					\varphi_\star
				\bigr)
			}
		\end{align*}
		where the last inequality uses the already proven \ref{thm:ErrorBound}.
		After suitably rearranging the sought inequality follows.
% 	\item\ref{thm:ErrorBound2}~
% 		Follows by combining \ref{thm:cost_dist} and \ref{thm:ErrorBound}.
% 	\item\ref{thm:LinDecrease}~
% 		From \eqref{eq:ProxIneq} with \(y=x_\star\) we have
% 	\begin{align*}
% 		\|\bar x-x_\star\|^2
% 	{}\leq{} &
% 		(1-\gamma\mu_f)\|x-x_\star\|^2
% 		{}-{}
% 		\underbracket{
% 			\gamma^2(1-\gamma L_f)\|\Res(x)\|^2
% 		}_{\ref{thm:ErrorBound2}}
% 		{}-{}
% 		2\gamma
% 		\bigl(
% 			\underbracket{
% 				\varphi(\bar x)
% 				{}-{}
% 				\varphi_\star
% 			}_{\ref{thm:cost_dist}}
% 		\bigr)
% 	\\
% 	{}\leq{} &
% 		(1-\gamma\mu_f)\|x-x_\star\|^2
% 		{}-{}
% 		\tfrac{
% 			(\gamma\mu_f)^2
% 			(1-\gamma L_f)
% 		}{
% 			1-\gamma\mu_f(2-\gamma L_f)
% 		}
% 		\|\bar x-x_\star\|^2
% 		{}-{}
% 		\gamma\mu_f
% 		\|\bar x-x_\star\|^2.
% 	\end{align*}
% 	Rearranging, we have that
% 	\(
% 		\|\bar x-x_\star\|^2
% 	{}\leq{}
% 		c\|x-x_\star\|^2
% 	\)
% 	where, denoted \(\kappa\coloneqq\nicefrac{L_f}{\mu_f}\geq 1\) the condition number of \(f\),
% 	\begin{align*}
% 		c
% 	{}={} &
% 		c(\gamma,\kappa)
% 	{}={}
% 		(1-\gamma\mu_f)
% 		\left(
% 			1
% 			{}+{}
% 			\tfrac{
% 				(\gamma\mu_f)^2
% 				(1-\gamma L_f)
% 			}{
% 				1-\gamma\mu_f(2-\gamma L_f)
% 			}
% 			{}+{}
% 			\gamma\mu_f
% 		\right)^{-1}
% 	\\
% 	{}={} &
% 		(1-\gamma\mu_f)
% 		\bigl(
% 			1
% 			{}-{}
% 			\gamma\mu_f
% 			\tfrac{
% 				1-\gamma\mu_f
% 			}{
% 				1-\gamma\mu_f+\gamma\mu_f\gamma L_f
% 				{}-{}
% 				(\gamma\mu_f)^2
% 			}
% 		\bigr)
% 	\\
% 	{}={} &
% 		(1-\xi)
% 		\bigl(
% 			1
% 			{}-{}
% 			\xi
% 			\tfrac{
% 				1-\xi
% 			}{
% 				1-\xi+(\kappa-1)\xi^2
% 			}
% 		\bigr)
% 	\end{align*}
	\qedhere
	\end{proofitemize}
% \end{appendixproof}
\end{proof}


==> TeX/pre_Preamble.tex <==
%% To avoid warnings, amsmath must be loaded before svmult class
	\RequirePackage{amsmath}


%% To solve warnings raised by color package, force loading xcolor rather than color.
%  This is done by redefining \RequirePackage; the original command is restored after
%  class declaration in TeX/Preamble.tex
	\PassOptionsToPackage{usenames,dvipsnames}{xcolor}
	\PassOptionsToPackage{appendix}{clevethm}
	\PassOptionsToPackage{noend}{algpseudocode}
	\let\OLDRequirePackage\RequirePackage
	\def\colorstring{color}%
	\renewcommand\RequirePackage[2][]{%
		\def\argstring{#2}%
		\ifx\colorstring\argstring\relax
			\OLDRequirePackage[#1]{xcolor}%
		\else
			\OLDRequirePackage[#1]{#2}%
		\fi
	}

